DAB-DETR: Dynamic Anchor Boxes are Better Queries for DETR

We present in this paper a novel query formulation using dynamic anchor boxes for DETR (DEtection TRansformer) and offer a deeper understanding of the role of queries in DETR. This new formulation directly uses box coordinates as queries in Transformer decoders and dynamically updates them layer-by-layer. Using box coordinates not only helps using explicit positional priors to improve the query-to-feature similarity and eliminate the slow training convergence issue in DETR, but also allows us to modulate the positional attention map using the box width and height information. Such a design makes it clear that queries in DETR can be implemented as performing soft ROI pooling layer-by-layer in a cascade manner. As a result, it leads to the best performance on MS-COCO benchmark among the DETR-like detection models under the same setting, e.g., AP 45.7\% using ResNet50-DC5 as backbone trained in 50 epochs. We also conducted extensive experiments to confirm our analysis and verify the effectiveness of our methods. Code is available at \url{https://github.com/SlongLiu/DAB-DETR}.

==> iclr2022/image_attn_decouple.tex <==
% \begin{figure}[t]
% \centering
% \subfigure{
% \begin{minipage}[t]{0.6\linewidth}
% \centering
% \includegraphics[width=\linewidth]{iclr2022/images/plot_decouple_attn.pdf}
% \caption{\small{Decoupled attention maps between queries and features. Positional attentions act like anchors to filter objects in certain regions.}}
% \label{fig:decouple_attn}
% \end{minipage}
% }%
% \subfigure{
% \begin{minipage}[t]{0.36\linewidth}
% \centering
% \includegraphics[width=\linewidth]{iclr2022/images/compare_detr_2d_4d_50.png}
% \caption{\small{Comparison of DETR, and our DAB-DETRs that learn 2D points and 4D boxes respectively.}}
% \label{fig:compare_2d_4d}
% \end{minipage}
% }%
% \end{figure}
\begin{figure}[t]
\centering
\includegraphics[width=0.4\linewidth]{iclr2022/images/plot_decouple_attn.pdf}
\caption{\small{Decoupled attention maps between queries and features.
    % The positional attentions are calculated by the lear
Positional attentions act like anchors to filter objects in certain regions.}}
\label{fig:decouple_attn}
\end{figure}

==> iclr2022/image_iter.tex <==
\begin{figure}[htbp]
\centering
\subfigure{
\begin{minipage}[t]{0.28\linewidth}

\centering
\includegraphics[width=\linewidth]{iclr2022/images/layer_0.png}
% \caption{initial anchor boxes.}
\end{minipage}
}%
\subfigure{
\begin{minipage}[t]{0.28\linewidth}
\centering
\includegraphics[width=\linewidth]{iclr2022/images/layer_1.png}
% \caption{anchor boxes after the first decoder.}
\end{minipage}
}%
\subfigure{
\begin{minipage}[t]{0.1\linewidth}
\centering
\vspace{-1.8cm}
$\rightarrow$
\end{minipage}
}%
\subfigure{
\begin{minipage}[t]{0.28\linewidth}
\centering
\includegraphics[width=\linewidth]{iclr2022/images/layer_6.png}
% \caption{predicted boxes.}
\end{minipage}
}%
\centering
\caption{{Layer-by-layer anchor box update. We plot the initial anchor boxes (left), anchor boxes after the first decoder layer (middle), and the output of the last decoder layer (right), respectively. The green boxes are ground truth annotations while red boxes are predictions of our model.} The results are obtained with the ResNet-50 backbone. More results are available in Appendix.
% \leizhang{which backbone?}.}\leizhang{you may provide visualizations for more images. If space is not allowed, put them in Appendix.}
}
\label{fig:iter_update}
\end{figure}
